Delay Optimization of Combinational Logic by And-Or Path Restructuring

We propose a dynamic programming algorithm that constructs delay-optimized circuits for alternating And-Or paths with prescribed input arrival times. Our algorithm fulfills best-known approximation guarantees and empirically outperforms earlier methods by exploring a significantly larger portion of the solution space. Our algorithm is the core of a new timing optimization framework that replaces critical paths of arbitrary length by logically equivalent realizations with less delay. Our framework allows revising early decisions on the logical structure of the netlist in a late step of an industrial physical design flow. Experiments demonstrate the effectiveness of our tool on 7nm real-world instances.

==> abstract_no_math.tex <==

We propose a timing optimization framework that replaces critical paths by logically
equivalent realizations with less delay.
Our framework allows to revise early decisions on the logical structure of the netlist
in late physical design.

The core routine of our framework is a new algorithm
that constructs delay-optimized circuits for alternating AND-OR paths
with prescribed input arrival times.
Our algorithm is a sophisticated dynamic program
which is a common generalization of the previously best approaches.
In contrast to all earlier methods,
we avoid fixing the structure of sub-solutions before deciding on how to combine them,
significantly expanding the solution space of the dynamic program.
Our algorithm provably fulfills best-known approximation guarantees,
and experiments show that in most cases it is considerably better than previous approaches.

The reduction to AND-OR path optimization allows us to optimize paths of arbitrary length in our logic restructuring framework.
The framework is applied successfully as a late step in an
industrial physical design flow.
Experiments demonstrate the effectiveness
of our tool on industrial 7nm instances.



==> abstract_sug.tex <==
We propose a timing optimization framework that replaces critical paths by logically
equivalent realizations with less delay.
Our framework allows to revise early decisions on the logical structure of the netlist
in late physical design.

The core routine of our framework is a new algorithm
that constructs delay-optimized circuits for alternating \aop{}s
with prescribed input arrival times.
Our algorithm is a sophisticated dynamic program
which is a common generalization of the previously best approaches.
In contrast to all earlier methods,
we avoid fixing the structure of sub-solutions before deciding on how to combine them,
significantly expanding the solution space of the dynamic program.
Our algorithm provably fulfills best-known approximation guarantees,
and experiments show that in most cases it is considerably better than previous approaches.

The reduction to \aop{} optimization allows us to optimize paths of arbitrary length in our logic restructuring framework.
The framework is applied successfully as a late step in an
industrial physical design flow.
Experiments demonstrate the effectiveness
of our tool on industrial 7nm instances.



==> smallest_instance.tex <==

\node[outer sep=0pt] (x0) at (0.5, 3.2){$x_0$};
\node[outer sep=0pt] (x1) at (1.5, 3.2){$x_1$};
\node[outer sep=0pt] (x2) at (2.5, 3.2){$x_2$};
\node[outer sep=0pt] (x3) at (3.5, 3.2){$x_3$};
\node[outer sep=0pt] (x4) at (4.5, 3.2){$x_4$};
\node[outer sep=0pt] (x5) at (5.5, 3.2){$x_5$};
\node[outer sep=0pt] (x6) at (6.5, 3.2){$x_6$};
\node[outer sep=0pt] (x7) at (7.5, 3.2){$x_7$};
\node[outer sep=0pt] (x8) at (8.5, 3.2){$x_8$};
\node[outer sep=0pt] (x9) at (9.5, 3.2){$x_9$};

\node[fill=red, outer sep=0pt, and gate US, draw, logic gate inputs=nn, rotate=270, thick] at (9,2) (and1){};
\draw[thick] (x9) -- (and1.input 1);
\draw[thick] (x8) -- (and1.input 2);

\node[fill=green, outer sep=0pt, or gate US, draw, logic gate inputs=nn, rotate=270, thick] at (8,1) (or1){};
\draw[thick] (and1.output) -- (or1.input 1);
\draw[thick] (x7) -- (or1.input 2);

\node[fill=red, outer sep=0pt, and gate US, draw, logic gate inputs=nn, rotate=270, thick] at (7,0) (and2){};
\draw[thick] (or1.output) -- (and2.input 1);
\draw[thick] (x6) -- (and2.input 2);

\node[fill=green, outer sep=0pt, or gate US, draw, logic gate inputs=nn, rotate=270, thick] at (6,-1) (or2){};
\draw[thick] (and2.output) -- (or2.input 1);
\draw[thick] (x5) -- (or2.input 2);

\node[fill=red, outer sep=0pt, and gate US, draw, logic gate inputs=nn, rotate=270, thick] at (5,-2) (and3){};
\draw[thick] (or2.output) -- (and3.input 1);
\draw[thick] (x4) -- (and3.input 2);

\node[fill=green, outer sep=0pt, or gate US, draw, logic gate inputs=nn, rotate=270, thick] at (4,-3) (or3){};
\draw[thick] (and3.output) -- (or3.input 1);
\draw[thick] (x3) -- (or3.input 2);

\node[fill=red, outer sep=0pt, and gate US, draw, logic gate inputs=nn, rotate=270, thick] at (3,-4) (and4){};
\draw[thick] (or3.output) -- (and4.input 1);
\draw[thick] (x2) -- (and4.input 2);

\node[fill=green, outer sep=0pt, or gate US, draw, logic gate inputs=nn, rotate=270, thick] at (2,-5) (or4){};
\draw[thick] (and4.output) -- (or4.input 1);
\draw[thick] (x1) -- (or4.input 2);

\node[fill=red, outer sep=0pt, and gate US, draw, logic gate inputs=nn, rotate=270, thick] at (1,-6) (and5){};
\draw[thick] (or4.output) -- (and5.input 1);
\draw[thick] (x0) -- (and5.input 2);

==> zwl.tex <==
\begin{table}
\setlength{\tabcolsep}{4pt}
\newcommand{\interrowspace}{.1cm}
\begin{tabular}{ llrrrr }
\toprule

Chip & Run & \multicolumn{1}{c}{WS [ps]} & \multicolumn{1}{c}{TS [ns]} & \multicolumn{1}{c}{Area}      & \multicolumn{1}{c}{\# Gates} \\
%      &     & \multicolumn{1}{c}{[ps]}        & \multicolumn{1}{c}{[ns]} & \multicolumn{1}{c}{[\%]} & \multicolumn{2}{c}{}               \\
\midrule

%
% Table body begin
%

\chipName{superblue1}  & init & \rmUkn{-152.9}  & \rmUkn{-103.4}  &                   & \rmUkn{1158946}  \\
                       & \BL  & \rmBtr{172.7}   & \rmBtr{-76.9}   & \rmEql{-0.17 \%}  & \rmEql{1159063}\vspace{\interrowspace}\\
\chipName{superblue3}  & init & \rmUkn{-56.1}   & \rmUkn{-71.1}   &                   & \rmUkn{1102025}\\
                       & \BL  & \rmBtr{105.9}   & \rmWrs{-76.0}   & \rmEql{-0.04 \%}  & \rmEql{1102020}\vspace{\interrowspace}\\
\chipName{superblue4}  & init & \rmUkn{1087.4}  & \rmUkn{-27.4}   &                   & \rmUkn{821051}   \\
                       & \BL  & \rmBtr{1435.9}  & \rmBtr{-24.8}   & \rmEql{-0.03 \%}  & \rmEql{821049}\vspace{\interrowspace}\\
\chipName{superblue5}  & init & \rmUkn{1063.1}  & \rmUkn{-3.2}    &                   & \rmUkn{997405}   \\
                       & \BL  & \rmBtr{1227.5}  & \rmBtr{-2.2}    & \rmEql{-0.06 \%}  & \rmEql{996071}\vspace{\interrowspace}\\
\chipName{superblue7}  & init & \rmUkn{477.8}   & \rmUkn{-30.4}   &                   & \rmUkn{2142822}  \\
                       & \BL  & \rmBtr{743.1}   & \rmBtr{-24.1}   & \rmEql{+0.01 \%}  & \rmEql{2142877}\vspace{\interrowspace}\\
\chipName{superblue10} & init & \rmUkn{1121.7}  & \rmUkn{-26.7}   &                   & \rmUkn{1574593}  \\
                       & \BL  & \rmBtr{1388.3}  & \rmBtr{-13.0}   & \rmEql{+0.02 \%}  & \rmEql{1574847}\vspace{\interrowspace}\\
\chipName{superblue16} & init & \rmUkn{1700.6}  & \rmUkn{0}       &                   & \rmUkn{995717}   \\
                       & \BL  & \rmEql{1700.6}  & \rmEql{0}       & \rmEql{-0.01 \%}  & \rmEql{995717}\vspace{\interrowspace}\\
\chipName{superblue18} & init & \rmUkn{1192.6}  & \rmUkn{-11.2}   &                   & \rmUkn{694391}   \\
                       & \BL  & \rmBtr{1350.7}  & \rmBtr{-11.1}   & \rmEql{-0.06 \%}  & \rmEql{694374}\vspace{\interrowspace}\\

%
% Table body end
%
\bottomrule
\end{tabular}
\caption{Performance on ICCAD 2015 benchmarks using a zero-wire-load timing model.}
\label{table-zwl}
\end{table}

